Owicki-Gries Reasoning for C11 Programs with Relaxed Dependencies (Extended Version)

Deductive verification techniques for C11 programs have advanced significantly in recent years with the development of operational semantics and associated logics for increasingly large fragments of C11. However, these semantics and logics have been developed in a restricted setting to avoid the thin-air-read problem. In this paper, we propose an operational semantics that leverages an intra-thread partial order (called semantic dependencies) induced by a recently developed denotational event-structure-based semantics. We prove that our operational semantics is sound and complete with respect to the denotational semantics. We present an associated logic that generalises a recent Owicki-Gries framework for RC11 (repaired C11), and demonstrate the use of this logic over several example proofs.

==> extensions.tex <==
\section{Extensions to the semantics}

\subsection{RMW}

Recalling that $\Sigma$ denotes the set of all possible C11 states and
$\W$ is the set of all writes (including updates), each step of the
event semantics is formalised by the transition relation
$\mathord{\strans{\ \ }_{\Pad}} \subseteq \Sigma \times \W_\bot \times
\TA \times \Sigma$ (see \reffig{fig:c11-opsem}), where we have
$\W_\bot = \W \cup \{\bot\}$ and $\bot \notin \W$. Again, we write
$\sigma \strans{w, e}_{\Pad} \sigma'$ for
$(\sigma, w, e, \sigma') \in \mathord{\strans{\ \ }_{\Pad}}$.

For each rule $\sigma \strans{w, e}_{\Pad} \sigma'$, $w$ is the
\emph{write being observed} by the event $e$. Strictly speaking, the
event semantics could be defined without the $w$. However, making this
observed write explicit is useful for the verification
(\refsec{sect:verif}).




\begin{figure}[t]
  \centering
  \small
  $ \inference[{\sc Read}] {a \in \{rd(x, n),
    rd^\mathsf{A}(x, n) \}  \quad  \loc(w) = x \quad \wrval(w)=n   \\
    w \in \OW_\sigma(t) \quad \ltrf' = \ltrf \cup
    \{(w,e)\}  \quad \ltmo' = \ltmo } {((D,
    \ltsb),\ltrf,\ltmo) \strans{w,e}_{\Pad} ((D, \ltsb) + e,\ltrf',\ltmo')}$
  \bigskip

  $ \inference[{\sc Write}] {% e = (g, a, t) \quad g \notin tags(D) \quad
    a \in \{ wr(x,n),
    wr^{\sf R}(x,n)\} \quad w \in \OW_\sigma(t) \backslash
    \CW_\sigma \\ \loc(w) = x \quad  \ltrf' = \ltrf \quad
    \ltmo' = \ltmo[w,e] % loc(e)
  }{((D,
    \ltsb),\ltrf,\ltmo) \strans{w, e}_{\Pad} ((D, \ltsb) + e,\ltrf',\ltmo')}$ \bigskip


  $\inference[{\sc RMW}] {% e = (g, a, t) \quad g \notin tags(D) \quad
    a = upd^{\sf
      RA}(x,m,n) 
    \quad w \in \OW_\sigma(t) \backslash \CW_\sigma \quad \loc(w)
    = x \\ \wrval(w)=m \quad \ltrf' = \ltrf \cup \{(w,e)\} \quad
    \ltmo' = \ltmo[w,e]} {((D,
    \ltsb),\ltrf,\ltmo) \strans{w,e}_{\Pad} ((D, \ltsb) +
    e,\ltrf',\ltmo')}$

  \caption{Event semantics assuming
    $\sigma = ((D, \ltsb),\ltrf,\ltmo)$, $e = (g, a, t)$  and $g \notin tags(D)$}
  \label{fig:c11-opsem-RMW}
\end{figure}

We now describe each of the rules in \reffig{fig:c11-opsem}. Executing
each event $e$ updates $(D, \ltsb)$ to:
\begin{align*} 
  (D, \ltsb) + e
  & =
    \left(\begin{array}[c]{@{}l@{}}
      D \cup \{e\}, 
      \ \ltsb \cup  (\{e' \in D  \mid \tid(e') \in \{\tid(e), 0\} \}
      \times \{e\} )
    \end{array}\right)
\end{align*} 
Thus, the initial writes are $\ltsb$-prior to every non-initialising
event.  Relations $\ltrf$ and $\ltmo$ are updated according to the
write events in $D$ that are observable to the thread executing the
given event. To this end, we must distinguish three sets of writes:
\emph{encountered writes} and \emph{observable writes}, which are
specific to each thread, and \emph{covered writes}, which are the set
of writes that are immediately followed, in reads-from order, by an
update event.

The set of \emph{encountered writes} are the writes that thread $t$ is
aware of (either directly or indirectly) in state
$\sigma=((D,\ltsb),\ltrf,\ltmo)$, and are given by:
\begin{align*}
  \observedWrites_\sigma(t) = \{w  \in \W \cap D \mid \exists e \in D.\
  \begin{array}[t]{@{}l@{}}
    \tid(e) = t \wedge {} 
    (w,e) \in \lteco^?; \lthb^? \}
  \end{array}
\end{align*}
where $R^?$ is the reflexive closure of relation $R$.  Thus, for each
$w \in \observedWrites_\sigma(t)$, there must exist an event $e$ of
thread $t$ such that $w$ is either $\lteco$- or $\lthb$- or
$\lteco ; \lthb$-prior to $e$. Note that $\observedWrites_\sigma(t) = \emptyset$ if the thread $t$ has not executed any actions; as soon as the thread executes its first action, we have $I \subseteq \observedWrites_\sigma(t)$. 

From these, we determine the \emph{observable writes}, which are the
writes that thread $t$ can observe in its next read. These are defined
as:
\begin{align*}
  \OW_\sigma(t) = \{w  \in \W \cap D  \mid \forall w' \in \observedWrites_\sigma(t).\ (w,w') \notin \ltmo\}
\end{align*}
Thus, observable writes are not succeeded by any encountered write in
modification order, i.e., the thread has not seen another write
overwriting the value being read.

Finally, to guarantee {\em atomicity} of the update events, there
cannot be any write operations (in modification order) between the
write that an update reads from and the write of the update itself. We
therefore define the set of \emph{covered writes} as follows:
\begin{align*}
  \CW_\sigma = \{w \in \W \cap D \mid \exists u \in \URA.\ (w,u) \in \ltrf\}   
\end{align*}


\subsection{While loops}


